Micro-CernVM: Slashing the Cost of Building and Deploying Virtual Machines

The traditional virtual machine building and and deployment process is centered around the virtual machine hard disk image. The packages comprising the VM operating system are carefully selected, hard disk images are built for a variety of different hypervisors, and images have to be distributed and decompressed in order to instantiate a virtual machine. Within the HEP community, the CernVM File System has been established in order to decouple the distribution from the experiment software from the building and distribution of the VM hard disk images. We show how to get rid of such pre-built hard disk images altogether. Due to the high requirements on POSIX compliance imposed by HEP application software, CernVM-FS can also be used to host and boot a Linux operating system. This allows the use of a tiny bootable CD image that comprises only a Linux kernel while the rest of the operating system is provided on demand by CernVM-FS. This approach speeds up the initial instantiation time and reduces virtual machine image sizes by an order of magnitude. Furthermore, security updates can be distributed instantaneously through CernVM-FS. By leveraging the fact that CernVM-FS is a versioning file system, a historic analysis environment can be easily re-spawned by selecting the corresponding CernVM-FS file system snapshot.

==> img/overlay.tex <==
%\documentclass[a4paper, 11pt]{article}\usepackage{tikz,ifthen}\usetikzlibrary{arrows,positioning,shapes,topaths,calc,fit,backgrounds,matrix,shadows}\begin{document}

\newsavebox{\tikzfilesystemovl}
\savebox{\tikzfilesystemovl}{
\begin{tikzpicture}
	[
		dirent/.style={
			circle,
			draw=green!50!black!50,
			fill=green!50!black!50,
			scale=0.35pt
		}
	]
	\node[dirent] (root) at (0,1.6) {};
	\node[dirent,red!50!black!50,fill=red!50!black!50] (d1) at (0.4, 1.2) {};
	\node[dirent] (d2) at (0.4, 0.8) {};
	\node[dirent,red!50!black!50,fill=red!50!black!50] (d21) at (0.8, 0.4) {};
	\node[dirent] (d22) at (0.8, 0) {};
	
	\draw (root) -- (0,1.2) -- (d1);
	\draw (0,1.2) -- (0,0.8) -- (d2) -- (0.4, 0.4) -- (d21);
	\draw (0.4,0.4) -- (0.4,0) -- (d22);
	\draw (0,0.8) -- (0,0);		
	
	\node at (-0.2,0.1) {\includegraphics[height=1cm]{img/folder}};
\end{tikzpicture}
}

\begin{tikzpicture}
	\tikzstyle{every node}=[font=\large]
	\colorlet{colrepo}{blue!50}
	\colorlet{colscratch}{red!40}
	\colorlet{colunion}{blue!50!black}

	\node[fill=colrepo, semitransparent, trapezium, trapezium left angle=30, trapezium right angle=-30, minimum width=9.5cm] (repository) {};
	\node[blue, anchor=south, xshift=0.5cm] at (repository.bottom side) {CernVM-FS Read-Only};
	
	\node[fill=colscratch, semitransparent, drop shadow, trapezium, trapezium left angle=30, trapezium right angle=-30, minimum width=9.25cm] (scratch) at ($(repository)+(0.75, 0.75)$) {};
	\node[red!80!black, anchor=south, xshift=0.5cm] at (scratch.bottom side) {Read/Write Scratch Area};
	
	\draw[colunion, ->, line width=1ex, rounded corners] (4,-0.5) -- node[fill=white] {\parbox{4cm}{\centering AUFS\\(Union File System)}} ++(0,-2) -- ++(-3.75,0);
	
	\node[draw, rectangle, very thick, colunion, rounded corners, minimum width=4.75cm, minimum height=2.75cm] at (-2.5, -3) {};
	\node[label={[colunion, label distance=-0.5cm]left:\parbox{2.5cm}{Read/Write\\ Interface}}] at (-1.25, -3) {\usebox{\tikzfilesystemovl}};
\end{tikzpicture}

%\end{document}
